Variational problems in thin elastic structures

For two different scenarios regarding thin elastic structures, described by 2d-F\"oppl-von K\'arm\'an plate models, we obtain energy scaling laws. Firstly, assuming the reference geometry being that of a singular excess-cone, we obtain fairly optimal upper- and lower energy bounds and we highlight how those bounds scale wrt. the thickness-parameter $h.$ Secondly, we consider the half sphere, while being indented by a thin object at the top and perpendicular to its surface. In this situation we provide an energy-scaling law, for radial symmetric admissible maps, this time, depending on $h$ and the indentation depth $d.$

==> MT12.tex <==
\subsection{Fully non linear plate model}
\begin{thm}\label{}
There are three constants $C_1,C_2,C_3>0$ s.t.
\begin{equation}
C_1h^2\log{\frac{1}{h}}+C_3h^2\le\inf\limits_{W^{2,2}(B_1,\R^3)} I_h(y)\le C_1 h^2\log{\frac{1}{h}}+C_2h^2
\label{eq:}
\end{equation}
where 
\begin{equation}\label{}
C_1=...,C_2=..., C_3=...?
\end{equation}
\end{thm}

\subsubsection{Upper-bound}
\begin{thm}\label{}
There are two constants $C_1,C_2>0$ s.t.
\begin{equation}
\inf\limits_{W^{2,2}(B_1,\R^3)}I_h(y)\le C_1 h^2\log{\frac{1}{h}}+C_2h^2
\label{eq:}
\end{equation}
where 
\begin{equation}\label{}
C_1=...,C_2=...?
\end{equation}
\end{thm}
First we prove that there exists an upper bound in the first place and that the constant $C_1$ can be written as the value of a minimization problem. Later on we will solve this problem to get the numerical value as claimed before.
\begin{lem}\label{}
There are two constants $C_1,C_2>0$ s.t.
\begin{equation}
\inf\limits_{W^{2,2}(B_1,\R^3)} I_h(y)\le C_1 h^2\log{\frac{1}{h}}+C_2h^2
\label{eq:}
\end{equation}
where 
\begin{equation}\label{}
C_1=\inf \limits_{\gamma\in C^2(S^1,S^2)}C_1(\gamma)=\frac{1}{\ln {2}}\inf \limits_{\tilde{y}=|x|\gamma(\xh)\atop \gamma\in C^2(S^1,S^2)}\int\limits_{B_1\setminus B_{1/2}}{|\grad^2 \tilde{y}|^2\; dx}.
\end{equation}
for $\tilde{y}=|x|\gamma(\xh)$ and some $\gamma$ s.t. $|\gamma|=1$ and $|\gamma'|=a>1,$ with $a=???$.\\
\end{lem}
%Note: a is defined s.t. \tilde{y} has the metric of the e-cone.

{\bf{Proof.}}
Let $\eta\in C^2[0,\infty)$  be a truncation satisfying $\eta(t)=t,$ if $t\ge 1$ and $\eta(t)=0$ for all $t\in [0,\frac{1}{2}]$.
Choose 
\begin{equation}
y_{h_*}(x)=h_*\eta\left(\frac{|x|}{h_*}\right)\gamma(\xh).
\end{equation}
Then we split up the Integral in a ball with Radius $h_*=|\log h|$?? In $B_{h_*}$ we have the estimates
$|\grad y_{h_*}|\le C$ and $|\grad^2 y_{h_*}|\le C/h_*$ and in $B_1\setminus B_{h_*}$ it holds $y_h=\tilde{y}$ and therefore $\grad^T y\grad^T y=g_e,$ this implies
\begin{eqnarray}\label{eq:}
I_h(y)=\int\limits_{B_{h_*}}{\left(|g_y-g_e|^2+h^2|\grad^2y|^2\right)\;dx}+\int\limits_{B_1\setminus B_{h_*}}{\left(|g_y-g_e|^2+h^2|\grad^2y|^2\right)\;dx}\\
\le Ch_*^2+Ch_*^2h_*^{-2}+h_*^2\int\limits_{B_1\setminus B_{h_*}}{|\grad^2y|^2\;dx}\\
\le C\int\limits_{B_{h_*}}{\left(|g_y-g_e|^2+h^2|\grad^2y|^2\right)\;dx}+h^2\int\limits_{B_1\setminus B_{h_*}}{|\grad^2y|^2\;dx}
\end{eqnarray}
For the last term we use a decomposition in dyadic ball rings and use the scaling property of $\tilde{y}:$

\begin{lem}\label{}
The Euler-Lagrange-Equation to the minimization problem
\begin{equation}
\frac{1}{\ln {2}}\inf \limits_{\tilde{y}=|x|\gamma(\xh)\atop \gamma\in C^2(S^1,S^2)}\int\limits_{B_1\setminus B_{1/2}}{|\grad^2 \tilde{y}|^2\; dx}.
\label{eq:}
\end{equation}
is given by
\begin{equation}\label{}
???.
\end{equation}
and the minimal value of the above integral is given by $????$.
\end{lem}
Note that this implies the claimed value of $C_1.$

{\bf{Proof.}} \\
Instead of looking at the above functional where functions of the form $\wt{W}:B_1\rightarrow S^2$ are considered we can go to polar coordinates and consider functions $\wt{y}:[0,1]\times [0,2\pi]\rightarrow S^2$ and the corresponding minimization problem

\begin{equation}\label{}
\inf \limits_{\wt{y}(r,t)=r\wt{\gamma}(t)} \frac{1}{\ln(2)}\int\limits_{B_1\setminus B_{1/2}}{|\grad^2 \wt{y}|^2\; dx}.
\end{equation}
where $ \wt{\gamma}\in \{\wt{\gamma}\in C^2([0,2\pi],S^2)|\wt{\gamma}(0)=\wt{\gamma}(2\pi)\}.$ 
Now we start by calculating the integral
\begin{eqnarray}
\frac{1}{\ln(2)}\int\limits_{B_1\setminus B_{1/2}}{|\grad^2 \wt{y}|^2\; dx}=\frac{1}{\ln(2)}\int\limits_{\frac{1}{2}}^1\int\limits_{0}^{2\pi}{\frac{1}{r}|\gamma+\gamma''|^2\; dt\;dr.}\\
=\int\limits_{0}^{2\pi}{|\gamma+\gamma''|^2\; dt}.
\label{eq:}
\end{eqnarray}
Again we can represent $\gamma$ in cylindrical coordinates:
$\gamma(t)=(\gamma_r(t)+1)e_r+\gamma_\vp(t)e_\vp+\gamma_3(t)e_3,$ for all $t\in[0,2\pi]$
and rewrite the above integral in terms of the real-valued functions $(\ga_r,\ga_\vp,\ga_3)$ instead of the vector-valued function $\gamma.$
The functional then takes the form
\begin{equation}
\int\limits_{0}^{2\pi}{(\ga_r''-2\ga_\vp')^2+(2\ga_r'+\ga_\vp'')^2+(\ga_3+\ga_3'')^2\; dt}.
\label{eq:}
\end{equation}
Furthermore the conditions $|\ga|^2=1$ and $|\ga'|^2=1+\Delta^2$
become
\begin{eqnarray}
(1+u)^2+v^2+w^2=1\\
(1+u+v')^2+(u'-v)^2+w'^2=1+\Delta^2
\label{eq:}
\end{eqnarray}
Combining these two and integrating leads to the constrains
\begin{eqnarray}
\int\limits_0^{2\pi}{(\Delta^2+\ga_3^2-\ga_3'^2-\ga_r'^2-\ga_\vp'^2-2(\ga_r+\ga_r\ga_\vp'-\ga_\vp\ga_r')\;dt}=0.
\label{eq:}
\end{eqnarray}


The Lagrangian is given by $\mathcal{L}(t;\ga_r,\ga_\vp,\ga_3;\ga_r',\ga_\vp',\ga_3';\ga_r'',\ga_\vp'',\ga_3'')=(\ga_r''-2\ga_\vp')^2+(2\ga_r'+\ga_\vp'')^2+(\ga_3+\ga_3'')^2+\lambda(\Delta^2+\ga_3^2-\ga_3'^2-\ga_r'^2-\ga_\vp'^2-2(\ga_r+\ga_r\ga_\vp'-\ga_\vp\ga_r'))$ Then the System of Euler-Lagrange-equations 
\begin{eqnarray}
\partial_{\ga_k}\mathcal{L}-\partial_t\partial_{\ga_k'}\mathcal{L}+\partial^2_t\partial_{\ga_k''}\mathcal{L}=0\;{\mbox{for}}\;k=r,\vp,3.
\label{eq:}
\end{eqnarray}
takes the form
\begin{eqnarray}
\ga_r^{(4)}+(\lambda-2)\ga_r''-4\ga_\vp'''-2\lambda\ga_\vp'-\lambda&=&0\label{eq:ELE1.2.1}\\
\ga_\vp^{(4)}+(\lambda-2)\ga_\vp''+4\ga_r'''+2\lambda\ga_r'&=&0\label{eq:ELE1.2.2}\\
\ga_3^{(4)}+(2+\lambda)\ga_3''+(1+\lambda)\ga_3&=&0
\label{eq:ELE1.2.3}
\end{eqnarray}
The last of this equations is the same as the one showing up in the Föppl-von Kármán model we studied before, therefore we know how to treat this equation, but we have to be a little bit careful, we can only use the general solution, but the values of the constants have (maybe) changed due to the different constraints. The general solution is again
\begin{equation}
\ga_3(t)=c_0\cos(t)+c_1\sin(t)+c_2\cos(\sqrt{1+\lambda}t)+c_3\sin(\sqrt{1+\lambda}t)
\label{eq:}
\end{equation}
for $\lambda\not=0$ and for $\lambda=0$
\begin{equation}
\ga(t)=c_0\cos(t)+c_1\sin(t)+c_2t\cos(t)+c_3t\sin(t).
\label{eq:}
\end{equation}
If we derive the 2nd equation and combine it with the first equation in a suitable way we get an expression for $\ga_r''$ depending only on derivatives of $\ga_\vp$
\begin{equation}
\label{eq:}
\end{equation}
By deriving this equation twice, we get similar formulas for $\ga_r'''$ and $\ga_r^{(4)}.$ Plugging this into the derivative of the 2nd equation from above we get an ODE of 7th order depending only on the function $\ga_\vp$:
\begin{eqnarray}
\ga_r^{(7)}+2(6+\lambda)\ga_r^{(5)}+(\lambda^2+12\lambda+4)\ga_r'''+4\lambda^2\ga_r'&=&0.\\
\ga_\vp^{(7)}+2(6+\lambda)\ga_\vp^{(5)}+(\lambda^2+12\lambda+4)\ga_\vp'''+4\lambda^2\ga_\vp'&=&-2\lambda^2.
\label{eq:}
\end{eqnarray}
The solution of the homogeneous linear differential equation is given by
\begin{equation}
\ga_r(t)=\sum\limits_{i=1}^3{\left(\frac{a_{i}}{\omega_i}\cos(\omega_i t)+\frac{a_{i}}{\omega_i}\cos(\omega_i t)\right)}+d_1
\label{eq:}
\end{equation}
The inhomogeneous one is solved by
\begin{equation}
\ga_\vp(t)=\sum\limits_{i=1}^3{\left(\frac{b_{i}}{\mu_i}\cos(\mu_i t)+\frac{b_{i}}{\mu_i}\cos(\mu_i t)\right)}+d_2
\label{eq:}
\end{equation}



\begin{eqnarray}
&&\int\limits_{0}^{2\pi}{(\ga_r''-2\ga_\vp')^2+(2\ga_r'+\ga_\vp'')^2+(\ga_3+\ga_3'')^2\; dt}\\
&=&\pi[(c_0^2+c_1^2)(n^2-1)^2+\sum\limits_{i=1}^3{((a_i^2+a_i'^2)(4+\omega_i^2)+(b_i^2+b_i'^2)(4+\mu_i^2))}]
\label{eq:}
\end{eqnarray}


\subsubsection{Lower-bound}
